Quantifying Perceptual Distortion of Adversarial Examples

Recent work has shown that additive threat models, which only permit the addition of bounded noise to the pixels of an image, are insufficient for fully capturing the space of imperceivable adversarial examples. For example, small rotations and spatial transformations can fool classifiers, remain imperceivable to humans, but have large additive distance from the original images. In this work, we leverage quantitative perceptual metrics like LPIPS and SSIM to define a novel threat model for adversarial attacks. To demonstrate the value of quantifying the perceptual distortion of adversarial examples, we present and employ a unifying framework fusing different attack styles. We first prove that our framework results in images that are unattainable by attack styles in isolation. We then perform adversarial training using attacks generated by our framework to demonstrate that networks are only robust to classes of adversarial perturbations they have been trained against, and combination attacks are stronger than any of their individual components. Finally, we experimentally demonstrate that our combined attacks retain the same perceptual distortion but induce far higher misclassification rates when compared against individual attacks.

==> tex_files/preliminaries.tex <==
In this section, we formally define what we mean by an adversarial example. For the purpose of this paper, we will only consider the domain of multiclass-classifiers. Similar ideas can be used for regression problems.

Letting $f$ be a multiclass-classifier that maps vectors in $\mathbb{R}^n$ to one of $C$ classes, we assume that $f$ is 


\subsection{Definitions and Notation}
Let $f$ be a multiclass-classifier that classifies real vectors with $n$ features into one of $C$ classes, i.e., $f:\mathbb{R}^n \rightarrow [C]$. Furthermore, suppose $f$ is trained on some distribution of real data $X$. We will refer to the input $n$-dimensional vectors as \emph{images}. We denote the power set by $\mathcal{P}(\cdot)$.

\begin{definition}[Threat Model]
A $\textbf{threat model}$ is a function $t : \mathcal{P}(\mathbb{R}^n) \rightarrow \mathcal{P}(\mathbb{R}^n)$ that takes as input a set of images and outputs a set of images that are valid perturbations of the input images.\footnote{Note that, traditionally, the input to a threat model is the singleton image for which we are generating adversarial examples and the output is the set of valid adversarial examples. We define it more generally over sets as we will compose various attacks, though we overload notation as such: $t(x) := t(\{x\})$.}
\end{definition}

\begin{definition}[Adversarial Attack]
An \textbf{adversarial attack} is a function $A: \mathbb{R}^n \rightarrow \mathbb{R}^n$ parameterized by both a classifier and a threat model mapping an image to an adversarial perturbation of the image such that for all $x\in \text{\emph{supp}}(X),\; A(x) \in t(x)$\footnote{This can be relaxed to a soft constraint such that we penalize if $A(x)$ is far from $t(x)$ under some notion of distance. However, in our work we model it as a hard constraint in all attacks.}. We say the attack is \textbf{successful} on image $x$ if $f(x) \neq f(A(x))$.
\end{definition}



\subsection{Assumptions}

Our work applies to the \emph{white box} setting. Under this assumption, the adversary has access to both the classifier $f$ and its gradients. This contrasts against the \emph{black box} setting, in which the adversary must generate attacks without using the classifier's gradients. Furthermore, we focus on untargeted adversarial attacks, though our work can be easily extended to the targeted setting.

\subsection{Problem Statement}
Under the above notation, the problem of finding adversarial examples can be framed as a decision problem: for a given classifier, threat model and input, $f, t$ and $x$ respectively, can we find an $A(\cdot)$ such that $f(A(x)) \neq f(x)$?

For example, under an $\linf$ threat model that allows an $\linf$ perturbation of $\eps$, the threat model is $t(x) \coloneqq \{x'~|~\norm{x-x'}_{\infty} \le \eps\}$. In this case, we can frame finding an adversarial attacks as an optimization problem \cite{Carlini2017-qm}:
$$
A(x) = \argmin_{\{x' \in t(x) ~|~ f(x) \neq f(x') \} } \mathcal{D}(x,x') 
$$

The ``success'' hard constraint can be softened by instead modeling that constraint as an error term and solving the Lagrangian problem as follows,
$$
A(x) = \argmin_{x' \in t(x)} \left(\mathcal{D}(x,x') + \lambda \ell_f(x, x')\right)
$$
for some $\lambda > 0$ and $\ell_f$ such that it is always 0 when $f(x) \neq f(x')$ and positive when $f(x) = f(x')$.

